ConstraintFlow: A DSL for Specification and Verification of Neural Network Analyses

We develop a declarative DSL - \cf - that can be used to specify Abstract Interpretation-based DNN certifiers. In \cf, programmers can easily define various existing and new abstract domains and transformers, all within just a few 10s of Lines of Code as opposed to 1000s of LOCs of existing libraries. We provide lightweight automatic verification, which can be used to ensure the over-approximation-based soundness of the certifier code written in \cf for arbitrary (but bounded) DNN architectures. Using this automated verification procedure, for the first time, we can verify the soundness of state-of-the-art DNN certifiers for arbitrary DNN architectures, all within a few minutes.

==> sections/overapproxneuron.tex <==
\begin{figure}
    \resizebox{\textwidth}{!}{
    \begin{tikzpicture}
        \node[circle, draw, minimum size=1cm] (node) at (0,0) {$n$};
        \node[right=0.5cm of node, yshift=0.6cm] (l) {$l  = -1$};
        \node[right=0.5cm of node, yshift=0.2cm] (u) {$u  = 3$};
        \node[right=0.5cm of node, yshift=-0.2cm] (L) {$L = 4 + 5n_1 + 6n_2$};
        \node[right=0.5cm of node, yshift=-0.6cm] (U) {$U = 3 - 2n_1$};
        \draw[dotted] (node.east) -- (l.west);
        \draw[dotted] (node.east) -- (u.west);
        \draw[dotted] (node.east) -- (L.west);
        \draw[dotted] (node.east) -- (U.west);

        \draw[dotted, ->] (-150:1.5) -- (node);
        \draw[dotted, <-] (-170:1.5) -- (node);
        \draw[dotted, ->] (-190:1.5) -- (node);
        \draw[dotted, <-] (-210:1.5) -- (node);

        \node[draw, above=of current bounding box, yshift=-0.7cm, xshift=-2cm] (name) {$\hh_C$};
        \node[draw, right=of name, xshift=6cm] {$\hh_S$};

        \begin{scope}[shift={(10cm,0cm)},local bounding box=f1box]
            \node (node) at (0,0) {$\prev$};
            
            \node[below=0cm of node.center, rotate=270, right=0.01cm] (node2) {$\mapsto$};
            \node[below=0.1cm of node2.center] (node3) {$\sval_2$};
            
            \node[left=0.5cm of node, yshift=0.6cm] (l) {$l  \mapsto \sval_7$};
            \node[left=0.5cm of node, yshift=0.2cm] (u) {$u  \mapsto \sval_8$};
            \node[left=0.5cm of node, yshift=-0.2cm] (L) {$L \mapsto \sval_9$};
            \node[left=0.5cm of node, yshift=-0.6cm] (U) {$U \mapsto \sval_{11} + \sval_{12}*\sval_{13} + \sval_{14}*\sval_{15}$};

            \draw[dotted] (node.west) -- (l.east);
            \draw[dotted] (node.west) -- (u.east);
            \draw[dotted] (node.west) -- (L.east);
            \draw[dotted] (node.west) -- (U.east);

            \draw[dotted, ->] (node) -- (0:1.5);
            
        \end{scope}
    \end{tikzpicture}
    }
    \caption{Parts of Concrete DNN $\hh_C$ and Symbolic DNN $\hh_S$}
    \label{fig:overapproxneuron}
\end{figure}
    

==> sections/symbolicdnn.tex <==
% \begin{figure}
% \resizebox{\textwidth}{!}{
% \begin{tikzpicture}
%     \begin{scope}[local bounding box=f1box]
%         \node (curr) at (0,0) {$\curr$};
%         \node[below=0cm of curr.center, rotate=270, right=0.01cm] (node2) {$\mapsto$};
%         \node[below=0.1cm of node2.center] (node3) {$\sval_1$};
%         \node[left=1.0cm of curr] (prev) {$\prev$};
%         \node[below=0cm of prev.center, rotate=270, right=0.01cm] (node4) {$\mapsto$};
%         \node[below=0.1cm of node4.center] (node5) {$\sval_2$};
%         \node[right=0.2cm of curr, yshift=0.6cm] (l) {$l \mapsto \sval_3$};
%         \node[right=0.2cm of curr, yshift=0.2cm] (u) {$u \mapsto \sval_4$};
%         \node[right=0.2cm of curr, yshift=-0.2cm] (L) {$L \mapsto \sval_5$};
%         \node[right=0.2cm of curr, yshift=-0.6cm] (U) {$U \mapsto \sval_6$};
    
%         \node[left=0.2cm of prev, yshift=0.6cm] (pl) {$\sval_7 \mapsfrom l$};
%         \node[left=0.2cm of prev, yshift=0.2cm] (pu) {$\sval_8 \mapsfrom u$};
%         \node[left=0.2cm of prev, yshift=-0.2cm] (pL) {$\sval_9 \mapsfrom L$};
%         \node[left=0.2cm of prev, yshift=-0.6cm] (pU) {$\sval_{10} \mapsfrom U$};
    
%         \node[below] at (current bounding box.south) {$\cc = (\sval_3 \leq \sval_1 \leq \sval_4) \wedge (\sval_5 \leq \sval_1 \leq \sval_6) \quad \cdots\prop(\curr)$};
%         \node[below] at (current bounding box.south) {$\wedge (\sval_7 \leq \sval_2 \leq \sval_8) \wedge (\sval_9 \leq \sval_2 \leq \sval_{10}) \quad \cdots \prop(\prev)$};
%         \node[below] at (current bounding box.south) {$\wedge (\sval_2 \leq 0 \implies \sval_1 = 0) \wedge (\sval_2 > 0 \implies \sval_1 = \sval_2) \quad \cdots \eta(\curr,\prev)$};
%         \node[below, yshift=-1.3cm] at (current bounding box.south) {(a)};
%         \draw[dotted] (curr.east) -- (l.west);
%         \draw[dotted] (curr.east) -- (u.west);
%         \draw[dotted] (curr.east) -- (L.west);
%         \draw[dotted] (curr.east) -- (U.west);
    
%         \draw[dotted] (prev.west) -- (pl.east);
%         \draw[dotted] (prev.west) -- (pu.east);
%         \draw[dotted] (prev.west) -- (pL.east);
%         \draw[dotted] (prev.west) -- (pU.east);
        
%         \draw[->] (prev.east) -- (curr.west) node[midway, above] {\relu};
%         \node[draw, above=of prev] {$\hh_S$};
%     \end{scope}
    
    
%     \begin{scope}[shift={(12.5cm,2cm)},local bounding box=f2box]
%         \node (curr) at (0,0) {$\curr$};
%         \node[below=0cm of curr.center, rotate=270, right=0.01cm] (node2) {$\mapsto$};
%         \node[below=0.1cm of node2.center] (node3) {$\sval_1$};
%         \node[left=1.0cm of curr] (prev) {$\prev$};
%         \node[below=0cm of prev.center, rotate=270, right=0.01cm] (node4) {$\mapsto$};
%         \node[below=0.1cm of node4.center] (node5) {$\sval_2$};
%         \node[right=0.2cm of curr, yshift=0.6cm] (l) {$l \mapsto \sval_3$};
%         \node[right=0.2cm of curr, yshift=0.2cm] (u) {$u \mapsto \sval_4$};
%         \node[right=0.2cm of curr, yshift=-0.2cm] (L) {$L \mapsto \sval_5$};
%         \node[right=0.2cm of curr, yshift=-0.6cm] (U) {$U \mapsto \sval_6$};
    
%         \node[left=0.2cm of prev, yshift=0.6cm] (pl) {$\sval_7 \mapsfrom l$};
%         \node[left=0.2cm of prev, yshift=0.2cm] (pu) {$\sval_8 \mapsfrom u$};
%         \node[left=0.2cm of prev, yshift=-0.2cm] (pL) {$\sval_9\mapsfrom L$};
%         \node[left=0.2cm of prev, yshift=-0.6cm] (pU) {$\sval_{11} + \sval_{12}*\textcolor{red}{\bm{\sval_{13}}} +  \sval_{14}*\textcolor{red}{\bm{\sval_{15}}} \mapsfrom U$};
    
%         \node[draw, above=of pU, yshift=-0.7cm] {$\hh'_S$};
%         \begin{scope}[shift={(-2cm,-2cm)},local bounding box=f3box]
%             \node (n2) at (0,0) {$n_2$};
%             \node[below=0cm of n2.center, rotate=270, right=0.01cm] (n2map) {$\mapsto$};
%             \node[below=0.1cm of n2map.center] (n2var) {$\textcolor{red}{\bm{\sval_{15}}}$};
%             \node[left=2.5cm of n2] (n1) {$n_1$};
%             \node[below=0cm of n1.center, rotate=270, right=0.01cm] (n1map) {$\mapsto$};
%             \node[below=0.1cm of n1map.center] (n1var) {$\textcolor{red}{\bm{\sval_{13}}}$};
            
            
        
%             \node[left=0.2cm of n1, yshift=0.6cm] (n1l) {$\sval_{16} \mapsfrom l$};
%             \node[left=0.2cm of n1, yshift=0.2cm] (n1u) {$\sval_{17} \mapsfrom u$};
%             \node[left=0.2cm of n1, yshift=-0.2cm] (n1L) {$\sval_{18} \mapsfrom L$};
%             \node[left=0.2cm of n1, yshift=-0.6cm] (n1U) {$\sval_{19} \mapsfrom U$};

%             \node[right=0.2cm of n2, yshift=0.6cm] (n2l) {$l \mapsto \sval_{20}$};
%             \node[right=0.2cm of n2, yshift=0.2cm] (n2u) {$u \mapsto \sval_{21}$};
%             \node[right=0.2cm of n2, yshift=-0.2cm] (n2L) {$L \mapsto \sval_{22}$};
%             \node[right=0.2cm of n2, yshift=-0.6cm] (n2U) {$U \mapsto \sval_{23}$};
    
%             \draw[dotted] (n2.east) -- (n2l.west);
%             \draw[dotted] (n2.east) -- (n2u.west);
%             \draw[dotted] (n2.east) -- (n2L.west);
%             \draw[dotted] (n2.east) -- (n2U.west);
        
%             \draw[dotted] (n1.west) -- (n1l.east);
%             \draw[dotted] (n1.west) -- (n1u.east);
%             \draw[dotted] (n1.west) -- (n1L.east);
%             \draw[dotted] (n1.west) -- (n1U.east);

%             \draw[red, dotted, <->] ($(pU.west) - (-2,0.2)$) -- ($(n1.north)$);
%             \draw[red, dotted, <->] ($(pU.west) - (-3.5,0.2)$) -- ($(n2.north west)$);
%         \end{scope}
    
%         \node[below] at (f2box.south) {$\cc' = (\sval_3 \leq \sval_1 \leq \sval_4) \wedge (\sval_5 \leq \sval_1 \leq \sval_6)  \quad \cdots\prop(\curr)$};
%         \node[below] at (f2box.south) {$\wedge (\sval_7 \leq \sval_2 \leq \sval_8) \wedge (\sval_9 \leq \sval_2 \leq (\sval_{11} + \sval_{12}*\sval_{13} +  \sval_{14}*\sval_{15}))  \quad \cdots\prop(\prev)$};
%         \node[below] at (f2box.south) {$\wedge (\sval_2 \leq 0 \implies \sval_1 = 0) \wedge (\sval_2 > 0 \implies \sval_1 = \sval_2)  \quad \cdots \eta(\curr, \prev)$};
%         \node[below] at (f2box.south) {$\wedge (\sval_{16} \leq \sval_{13} \leq \sval_{17}) \wedge (\sval_{18} \leq \sval_{13} \leq \sval_{19})  \quad \cdots\prop(n_1)$};
%         \node[below] at (f2box.south) {$\wedge (\sval_{20} \leq \sval_{15} \leq \sval_{21}) \wedge (\sval_{22} \leq \sval_{15} \leq \sval_{23})  \quad \cdots\prop(n_2)$};
%         \node[below, yshift=-0.23cm] at (f2box.south) {(b)};
%         \draw[dotted] (curr.east) -- (l.west);
%         \draw[dotted] (curr.east) -- (u.west);
%         \draw[dotted] (curr.east) -- (L.west);
%         \draw[dotted] (curr.east) -- (U.west);
    
%         \draw[dotted] (prev.west) -- (pl.east);
%         \draw[dotted] (prev.west) -- (pu.east);
%         \draw[dotted] (prev.west) -- (pL.east);
%         \draw[dotted] (prev.west) -- (pU.east);
        
%         \draw[->] (prev.east) -- (curr.west) node[midway, above] {\relu};
%     \end{scope}
    
%     \node at ($(f1box.east)!0.2!(f2box.west)$) {\mbox{\Huge $ \rightarrow$ }};
% \end{tikzpicture}
% }
% % \captionof{figure}{Symbolic DNN creation and Expansion}
% % \label{fig:symbolicdnn}
% \caption{Symbolic DNN creation and expansion for DeepPoly. $\prop(n) \equiv (l \leq n \leq u) \wedge (L \leq n \leq U)$
% % , where the property $\prop$ is that for each neuron $n$, $(l \leq n \leq u) \wedge (L \leq n \leq U)$ holds.
% }
%     \label{fig:symbolicdnn}
% \end{figure}


\begin{figure}
\resizebox{\textwidth}{!}{
\begin{tikzpicture}
    \begin{scope}[local bounding box=f1box]
        \node (curr) at (0,0) {$\curr$};
        \node[below=0cm of curr.center, rotate=270, right=0.01cm] (node2) {$\mapsto$};
        \node[below=0.1cm of node2.center] (node3) {$\sval_c$};
        \node[left=1.0cm of curr] (prev) {$\prev$};
        \node[below=0cm of prev.center, rotate=270, right=0.01cm] (node4) {$\mapsto$};
        \node[below=0.1cm of node4.center] (node5) {$\sval_p$};
        \node[right=0.4cm of curr, yshift=0.9cm] (l) {$l \mapsto \sval_c^l$};
        \node[right=0.4cm of curr, yshift=0.3cm] (u) {$u \mapsto \sval_c^u$};
        \node[right=0.4cm of curr, yshift=-0.3cm] (L) {$L \mapsto \sval_c^L$};
        \node[right=0.4cm of curr, yshift=-0.9cm] (U) {$U \mapsto \sval_c^U$};
        \node[left=0.4cm of prev, yshift=0.9cm] (pl) {$\sval_p^l \mapsfrom l$};
        \node[left=0.4cm of prev, yshift=0.3cm] (pu) {$\sval_p^u \mapsfrom u$};
        \node[left=0.4cm of prev, yshift=-0.3cm] (pL) {$\sval_p^L \mapsfrom L$};
        \node[left=0.4cm of prev, yshift=-0.9cm] (pU) {$\sval_p^U \mapsfrom U$};

        \node[below] at (current bounding box.south) {};
        \node[below] at (current bounding box.south) {};
        \node[below] at (current bounding box.south) {$\prop(\curr) = (\sval_c^l \leq \sval_c \leq \sval_c^u) \wedge (\sval_c^L \leq \sval_c \leq \sval_c^U)$};
        \node[below] at (current bounding box.south) {$\prop(\prev) =  (\sval_p^l \leq \sval_p \leq \sval_p^u) \wedge (\sval_p^L \leq \sval_p \leq \sval_p^U) $};
        \node[below] at (current bounding box.south) {$\cc_\eta =  (\sval_2 \leq 0 \implies \sval_1 = 0) \wedge (\sval_p > 0 \implies \sval_c = \sval_p)$};
        \node[below] at (current bounding box.south) {$\cc = \prop(\curr) \wedge \prop(\prev) \wedge \cc_\eta$};
        \node[below, yshift=-0.3cm] at (f1box.south) {(a)};
        \draw[dotted] (curr.east) -- (l.west);
        \draw[dotted] (curr.east) -- (u.west);
        \draw[dotted] (curr.east) -- (L.west);
        \draw[dotted] (curr.east) -- (U.west);
    
        \draw[dotted] (prev.west) -- (pl.east);
        \draw[dotted] (prev.west) -- (pu.east);
        \draw[dotted] (prev.west) -- (pL.east);
        \draw[dotted] (prev.west) -- (pU.east);
        
        \draw[->] (prev.east) -- (curr.west) node[midway, above] {\relu};
        \node[draw, above=of prev] {$\hh_S$};
    \end{scope}
    
    
    \begin{scope}[shift={(12.5cm,1.0cm)},local bounding box=f2box]
        \node (curr) at (0,0) {$\curr$};
        \node[below=0cm of curr.center, rotate=270, right=0.01cm] (node2) {$\mapsto$};
        \node[below=0.1cm of node2.center] (node3) {$\sval_1$};
        \node[left=1.0cm of curr] (prev) {$\prev$};
        \node[below=0cm of prev.center, rotate=270, right=0.01cm] (node4) {$\mapsto$};
        \node[below=0.1cm of node4.center] (node5) {$\sval_2$};
        \node[right=0.4cm of curr, yshift=0.9cm] (l) {$l \mapsto \sval_c^l$};
        \node[right=0.4cm of curr, yshift=0.3cm] (u) {$u \mapsto \sval_c^u$};
        \node[right=0.4cm of curr, yshift=-0.3cm] (L) {$L \mapsto \sval_c^L$};
        \node[right=0.4cm of curr, yshift=-0.9cm] (U) {$U \mapsto \sval_c^U$};
    
        \node[left=0.4cm of prev, yshift=0.9cm] (pl) {$\sval_p^l \mapsfrom l$};
        \node[left=0.4cm of prev, yshift=0.3cm] (pu) {$\sval_p^u \mapsfrom u$};
        \node[left=0.4cm of prev, yshift=-0.3cm] (pL) {$\sval_p^L \mapsfrom L$};
        \node[left=0.4cm of prev, yshift=-0.9cm] (pU) {$\sval_r^1 + \sval_r^2*\textcolor{red}{\bm{\sval_{n_1}}} +  \sval_r^3*\textcolor{red}{\bm{\sval_{n_2}}} \mapsfrom U$};
    
        \node[draw, above=of pU, yshift=-0.7cm] {$\hh'_S$};
        \begin{scope}[shift={(-2cm,-2.5cm)},local bounding box=f3box]
            \node (n2) at (0,0) {$n_2$};
            \node[below=0cm of n2.center, rotate=270, right=0.01cm] (n2map) {$\mapsto$};
            \node[below=0.1cm of n2map.center] (n2var) {$\textcolor{red}{\bm{\sval_{n_2}}}$};
            \node[left=2.5cm of n2] (n1) {$n_1$};
            \node[below=0cm of n1.center, rotate=270, right=0.01cm] (n1map) {$\mapsto$};
            \node[below=0.1cm of n1map.center] (n1var) {$\textcolor{red}{\bm{\sval_{n_1}}}$};
            
            
        
            \node[left=0.4cm of n1, yshift=0.9cm] (n1l) {$\sval_{n_1}^l \mapsfrom l$};
            \node[left=0.4cm of n1, yshift=0.3cm] (n1u) {$\sval_{n_1}^u \mapsfrom u$};
            \node[left=0.4cm of n1, yshift=-0.3cm] (n1L) {$\sval_{n_1}^L \mapsfrom L$};
            \node[left=0.4cm of n1, yshift=-0.9cm] (n1U) {$\sval_{n_1}^U \mapsfrom U$};

            \node[right=0.4cm of n2, yshift=0.9cm] (n2l) {$l \mapsto \sval_{n_2}^l$};
            \node[right=0.4cm of n2, yshift=0.3cm] (n2u) {$u \mapsto \sval_{n_2}^u$};
            \node[right=0.4cm of n2, yshift=-0.3cm] (n2L) {$L \mapsto \sval_{n_2}^L$};
            \node[right=0.4cm of n2, yshift=-0.9cm] (n2U) {$U \mapsto \sval_{n_2}^U$};
    
            \draw[dotted] (n2.east) -- (n2l.west);
            \draw[dotted] (n2.east) -- (n2u.west);
            \draw[dotted] (n2.east) -- (n2L.west);
            \draw[dotted] (n2.east) -- (n2U.west);
        
            \draw[dotted] (n1.west) -- (n1l.east);
            \draw[dotted] (n1.west) -- (n1u.east);
            \draw[dotted] (n1.west) -- (n1L.east);
            \draw[dotted] (n1.west) -- (n1U.east);

            \draw[red, dotted, <->] ($(pU.west) - (-2,0.2)$) -- ($(n1.north)$);
            \draw[red, dotted, <->] ($(pU.west) - (-3.5,0.2)$) -- ($(n2.north west)$);
        \end{scope}
    

        \node[below] at (f2box.south) {};
        \node[below] at (f2box.south) {};
        \node[below] at (f2box.south) {$\prop(\prev) = (\sval_p^l \leq \sval_p \leq \sval_p^u) \wedge (\sval_p^L \leq \sval_2 \leq (\sval_r^1 + \sval_r^2*\sval_{n_1} +  \sval_r^3*\sval_{n_2}))$};
        \node[below] at (f2box.south) {$\cc = \prop(\curr) \wedge \prop(\prev) \wedge \cc_\eta \wedge \prop(n_1) \wedge \prop(n_2)$};
        \node[below, yshift=-0.23cm] at (f2box.south) {(b)};
        \draw[dotted] (curr.east) -- (l.west);
        \draw[dotted] (curr.east) -- (u.west);
        \draw[dotted] (curr.east) -- (L.west);
        \draw[dotted] (curr.east) -- (U.west);
    
        \draw[dotted] (prev.west) -- (pl.east);
        \draw[dotted] (prev.west) -- (pu.east);
        \draw[dotted] (prev.west) -- (pL.east);
        \draw[dotted] (prev.west) -- (pU.east);
        
        \draw[->] (prev.east) -- (curr.west) node[midway, above] {\relu};
    \end{scope}
    
    \node at ($(f1box.east)!0.45!(f2box.west)$) {\mbox{\Huge $ \rightarrow$ }};
\end{tikzpicture}
}
% \captionof{figure}{Symbolic DNN creation and Expansion}
% \label{fig:symbolicdnn}
\caption{Symbolic DNN creation and expansion for DeepPoly. $\prop(n) \equiv (l \leq n \leq u) \wedge (L \leq n \leq U)$
% , where the property $\prop$ is that for each neuron $n$, $(l \leq n \leq u) \wedge (L \leq n \leq U)$ holds.
}
    \label{fig:symbolicdnn}
\end{figure}



